Recurrent networks improve neural response prediction and provide insights into underlying cortical circuits

Feedforward CNN models have proven themselves in recent years as state-of-the-art models for predicting single-neuron responses to natural images in early visual cortical neurons. In this paper, we extend these models with recurrent convolutional layers, reflecting the well-known massive recurrence in the cortex, and show robust increases in predictive performance over feedforward models across thousands of hyperparameter combinations in three datasets of macaque V1 and V2 single-neuron responses. We propose the recurrent circuit can be conceptualized as a form of ensemble computing, with each iteration generating more effective feedforward paths of various path lengths to allow a combination of solutions in the final approximation. The statistics of the paths in the ensemble provide insights to the differential performance increases among our recurrent models. We also assess whether the recurrent circuits learned for neural response prediction can be related to cortical circuits. We find that the hidden units in the recurrent circuits of the appropriate models, when trained on long-duration wide-field image presentations, exhibit similar temporal response dynamics and classical contextual modulations as observed in V1 neurons. This work provides insights to the computational rationale of recurrent circuits and suggests that neural response prediction could be useful for characterizing the recurrent neural circuits in the visual cortex.

==> discussion.tex <==
\section{Discussion}

% \todo{it's currently just a sketch}

% % \begin{enumerate}
% %     \item Demonstrated that recurrent models robustly outperformed similarly-sized feed-forward models, for neural response modeling of early visual areas.
% %     \item Proposed a novel approach to understand the recurrent computation as an multi-path ensemble, and demonstrated the correlation between model performance and two multi-path ensemble characteristics.
% % \end{enumerate}

% \begin{enumerate}
%     \item Recurrent as a computation mechanism vs.\@ recurrent circuits in the brain
%     \item Significance of multi-path framework --- connecting recurrent networks to ensemble learning literature.
%     \item future work -- modeling PSTH, checking results on non neural data and other areas, etc.
%     \item an expanded version of introduction.
% \end{enumerate}

\subsection{Key contributions of the study}
\label{nips2021:discussion:contribution}

By training tens of thousands of models on multiple neural data sets and employing a novel method that reformulates recurrent models as multi-path ensemble models, we have made the following contributions to the research of early visual areas and recurrent models.

Recurrent models could predict neural responses of early visual areas better than typical feed-forward models with matched hyperparameters and model sizes, especially when training data were less and the model size was larger. We show the relevant experimental results in detail in Section~\ref{results:datadriven_models} with a comprehensive comparison between recurrent models and feed-forward models trained under tens of thousands of settings, with different data sets, different amounts of training data, and different model hyperparameters (Section~\ref{nips2021:method:implementation-details:hyperparameters}). Overall, recurrent models outperformed feed-forward ones of matched size and hyperparameters almost consistently regardless of the setting, with some small differences for models with different numbers of layers and different readout modes (Section~\ref{nips2021:results:datadriven_models:overall_epilogue}). While the performance advantage of recurrent models over feed-forward ones was consistent, the magnitude of the advantage was larger under larger model size and less training data (Section~\ref{nips2021:results:datadriven_models:per_model_size}); in other words, recurrent models showed more advantage over feed-forward ones when the amount of training data per model parameter was less. While it will be certainly too speculative to claim that the architecture of our recurrent models can be mapped to neural circuitry of the brain faithfully, it's likely that our recurrent models captured some of the fundamental computational principles of the visual areas as a model prior that helps neural data prediction under less data.

The performance advantage of the recurrent model over the feed-forward one can be attributed to the former's compact and implicit multi-path ensemble that allows approximating the complex function underlying recurrent biological circuits with efficiency. We established the observation in two steps. First, we reformulated recurrent models as models with multiple feed-forward paths with shared parameters (Section~\ref{results:analysis:ensemble}); thus we were able to compare recurrent models and feed-forward models in a unified framework, with feed-forward models being degenerate multi-path models. Second, we compared feed-forward models and recurrent models using two key characteristics of their multi-path ensembles---average path length and path diversity (Section~\ref{results:analysis:length_and_diversity})---and found there was arguably a positive correlation between the path diversity of recurrent models and their performance advantage over feed-forward models (Section~\ref{results:analysis:length_and_diversity:length}). The recurrent computation information flow in a recurrent model implicitly defines a compact multi-path ensemble with shared parameters across paths (Figure~\ref{fig:results:depth_analysis:schema}); we propose that such compact multi-path ensemble allows approximating the complex function underlying recurrent biological circuits with more flexibility compared to feed-forward model matched in model size and hyperparameters. The usefulness of multi-path ensemble in neural data prediction could be due to the inherent advantage of ensemble models for machine learning \citep{Bishop:2006vk}, or due to some similarity between multi-path architectures and neural circuits, or due to a bit of both.


A balance of short and long paths in the ensemble is necessary for the recurrent model to achieve the best performance; on our data sets, models with more relative weights on shorter paths tended to perform better than models with more relative weights on longer paths. We established the observations by comparing different readout modes (Section~\ref{method:new:readout}) in terms of their multi-path ensembles. In particular, we found that better performing readout modes have their path length distribution more concentrated at shorter paths (Figure~\ref{fig:results:both:per_layer:diversity_vs_depth}) and removing shorter paths had more impact on the performance than removing longer paths in an ablation study (Figures~\ref{fig:results:8k:ablation7},\ref{fig:results:tang:ablation7}). The relative importance of shorter paths over longer ones might be data set- and task-dependent and requires further investigation. For recurrent models, different readout modes essentially represent different weight assignments to intermediate outputs at different iterations (Section~\ref{method:new:readout}); our exploration of different readout modes show that the ``vanilla'' weight assignment, or \texttt{no-avg} readout mode, performed much worse compared to other readout modes; the comparison of different readout modes in terms of performance metrics and multi-path ensembles shows that a balance of early and late information across iterations, or equivalently a balance of short and paths in the corresponding multi-path ensemble, is necessary for the recurrent model to achieve the best performance.


The novel method that reformulates recurrent models as multi-path ensemble models  provides a new perspective to understand recurrent models and connect recurrent models to the existing literature on ensemble models in the machine learning community. The key idea behind the reformulation method is that the complex information flow in recurrent computation can be approximated as a summation of multiple feed-forward paths with shared parameters (Sections~\ref{results:analysis:ensemble}). While the reformulation method is approximate by nature, the approximation was accurate enough in practice (Section~\ref{results:analysis:ensemble}) and we successfully explained the differences between recurrent models and feed-forward models as well as the differences among recurrent models by comparing the models' multi-path ensembles. It will be interesting to check the accuracy of our reformulation method in other machine learning tasks involving recurrent models or multi-path models with shared information flow among paths; understanding these complex models as simpler models summing over multiple paths can enable alternative model dissection and ablation methods for better understanding the merits of those complex models. For example, in many architecture search studies for recurrent networks \citep{DBLP:conf/iclr/CollinsSS17,DBLP:journals/corr/GreffSKSS15}, authors mostly try to justify some architectures over others using performance metrics alone; it will be interesting to apply our reformulation methods to those different architectures and see if different architectures also yield different multi-path ensembles. In addition, our reformulation method and analysis techniques can be applied to those recurrent models performing well in computer vision tasks \citep{nayebi2018task,DBLP:conf/nips/KubiliusSHMRIKB19,DBLP:conf/nips/HanWZFCL18}; these studies typically have little or no explanation on the performance advantage of recurrent models from a computational perspective and the authors often justify recurrent models by the abundance of recurrent connections in the brain \citep{10.1093/cercor/1.1.1-a}; our reformulation method might reveal additional insights on the performance advantage of recurrent models.


\subsection{Differences and relationships with relevant studies}

\subsubsection{Modeling temporal dynamics versus mean firing rates}
\label{nips2021:discussion:relationship:dynamics}
Most studies on visual areas involving recurrent models have tried to model temporal dynamics of neural data \citep{10.1371/journal.pcbi.1008215,Kietzmann21854,nayebi2018task,DBLP:conf/nips/KubiliusSHMRIKB19}, whereas our study trained recurrent models to predict average firing rates instead of temporal dynamics of visual neurons. We chose to model average firing rates because we wanted to know in addition to modeling temporal dynamics, whether there is additional benefit of using recurrent models for neural data modeling; after all, by construction feed-forward models are bound to perform worse for modeling temporal dynamics. Our study demonstrated the superiority of recurrent models in a more competitive setting where feed-forward models are more likely to perform well compared to modeling temporal dynamics. Our results on neural prediction are conceptually consistent with many computer vision-oriented studies \citep{nayebi2018task,DBLP:conf/nips/KubiliusSHMRIKB19,DBLP:conf/nips/HanWZFCL18,7298958} who have demonstrated that recurrent models can outperform feed-forward ones in static image classification tasks which do not involve explicit temporal dynamics. In many of these studies as well as ours, the internal dynamics of these models trained on  tasks without explicit temporal dynamics could be useful for modeling neurophysiological data or effects involving temporal dynamics; in \citet{nayebi2018task,DBLP:conf/nips/KubiliusSHMRIKB19}, the internal model dynamics have been reported to resemble actual monkey IT population dynamics; in our study (to be described later in Section~\ref{nips2021:discussion:relationship:existing_work}), the internal model dynamics exhibited longitudinal facilitation and lateral suppression of oriented bars \citep{Kapadia12073} as well as reduction in orientation bandwidths and spatial frequency bandwidths over time \citep{ringach1997dynamics,Bredfeldt1976}. The above results of using internal dynamics learned from static tasks to model temporal dynamics of neurophysiological data and effects suggest that there might be some general benefit about recurrent modeling regardless of tasks. 


\subsubsection{Existing work on modeling early visual areas}
\label{nips2021:discussion:relationship:existing_work}

Neural network-like models have long been used to model neural responses of early visual areas. Before the wide adoption of deep learning techniques, \citet{David:2005fi} tried to predict V1 neural responses using a fully connected layer followed by ReLU activation layer; \citet{Prenger:2004gp} modeled V1 neural data using more traditional multi-layer fully connected neural networks with sigmoid activation layers; \citet{Lau25062002} used neural networks to model and understand complex cells of V1; generalized linear models (GLMs) \citep{Pillow:2008bo,DBLP:conf/nips/KellySKL10}, subunit models \citep{Vintch14829}, nested GLMs \citep{McFarland:2013jr}, sparse deep belief nets for V2 \citep{DBLP:conf/nips/LeeEN07}, and boosting-based linear combinations of V1 models \citep{Willmore2102} can all be formulated as neural networks with specific network architecture designs and/or optimization techniques. In recent years, convolutional neural networks (CNNs) and its extensions have achieved great success for modeling early visual areas \citep{10.1371/journal.pcbi.1006897,DBLP:conf/nips/KlindtEEB17,Zhang2019,DBLP:conf/iclr/EckerSFFCWCRTB19}. Our study extends the above CNN work by applying recurrent CNNs to neural modeling tasks; more important, our novel reformulation method based on multi-path ensembles provides insights into the performance advantage of recurrent models.

While our study is one of the earliest ones to introduce lateral recurrent connections into CNNs for predicting mean firing rates of neurons in early visual areas, alternative mechanisms can introduce lateral connections to the model. Notable alternative mechanisms include  divisive normalization \citep{Carandini:2005kw} and dynamical system implementations of sparse coding \citep{DBLP:journals/neco/RozellJBO08,Zhu:2013fi,King:2013jp}. All of these mechanisms might be implementing similar underlying computational principles of the brain, as all these models are able to reproduce many neurophysiological phenomena associated with recurrent circuits. Preliminary results in \citet{halcosyne2021} showed that the internal model dynamics of our recurrent models exhibited longitudinal facilitation and lateral suppression of oriented bars \citep{Kapadia12073} as well as reduction in orientation bandwidths and spatial frequency bandwidths over time \citep{ringach1997dynamics,Bredfeldt1976}; models incorporating divisive normalization and sparse coding mechanisms are able to explain many non-classical receptive field effects of V1 neurons as well \citep{Carandini:2005kw,Zhu:2013fi}; in addition, divisive normalization mechanims can be incorporated into CNNs, with improved model interpretability and little loss in performance \citep{Burg767285}.


\subsubsection{Existing work connecting recurrent models and ensemble models}

There have been relatively few studies connecting recurrent models to multi-path ensemble models in the deep learning context. For ResNets, \citet{DBLP:journals/corr/LiaoP16} have pointed out the equivalence between a specific type of recurrent networks with weight-tied ResNets, and \citet{DBLP:conf/nips/ChenRBD18} formulate deep weight-tied ResNets as approximating the dynamics of continuous recurrent models specified in ordinary differential equations. To the best of our knowledge, there is no work explicitly connecting recurrent models to multi-path ensemble models in general. The most similar work to ours is probably \citet{DBLP:conf/nips/ZhangWCLMSB16}, which characterizes recurrent models in terms of some architectural complexity measures (feed-forward depth, recurrent depth, and recurrent skip coeffcient) motivated by graph theory and quantified the relationship between performance and these complexity measures. While conceptually similar, our work differs from \citet{DBLP:conf/nips/ZhangWCLMSB16} in two important aspects. First,  complexity measures in \citet{DBLP:conf/nips/ZhangWCLMSB16} are entirely based on model architecture hyperparameters, whereas our measures of the recurrent model's multi-path ensemble depend on both model hyperparameters as well as learned model parameters; second, \citet{DBLP:conf/nips/ZhangWCLMSB16} have developed their measures in the context of sequence modeling where both inputs and outputs of the task are variable-sized sequences, whereas we developed our measures of the multi-path ensemble for tasks with fixed-sized input and output.

\subsubsection{Alternative methods to deeply understand recurrent networks}
\label{nips2021:discussion:relationship:recurrent_deep_understanding}

In the deep learning community, recurrent networks have often been analyzed in a less rigorous fashion. For example, the practical performance advantage of gated recurrent networks, such as LSTM \citep{DBLP:journals/neco/HochreiterS97} and GRU \citep{DBLP:journals/corr/ChoMGBSB14}, over vanilla RNNs have often been attributed to the gate units' ability to alleviate gradient vanishing \cite{Goodfellow:2016wc}; in addition, various kinds of recurrent model hyperparameter grid search have been performed for recurrent networks to find and justify the best architectures for certain tasks \citep{DBLP:conf/iclr/CollinsSS17,DBLP:journals/corr/GreffSKSS15}. Certain types of recurrent models have been deeply analyzed in alternative ways.  \citet{DBLP:journals/neco/HintonOT06} have proved that an infinite logistic belief net with tied weights is equivalent to a restricted Boltzmann machine \citep{Hinton504}; in a more relevant study, \citet{DBLP:conf/nips/BaiKK19} have found that modern weight-tied deep recurrent networks in NLP tasks converge to a fixed point of the recurrent dynamics.

While our approach to understand recurrent models as multi-path ensembles succeeded in explaining the differences among recurrent and feed-forward models (Section~\ref{results:analysis:length_and_diversity}), we also explored whether the empirical observations about the convergence of recurrent models made in \citet{DBLP:conf/nips/BaiKK19} were applicable to our models. It turned out we failed to find any convergence to a fixed point for the internal dynamics of our models. The failure might be due to two reasons. First, the empirical  observations about convergence in \citet{DBLP:conf/nips/BaiKK19} probably only apply when the model dynamics is strictly recurrent, whereas our models actually follows a semi-recurrent dynamics with shared convolutional layers and independent normalization layers (Sections~\ref{nips2021:discussions:limitation:strict_recurrent},\ref{appendix:model_math:new}). Second, following the practice in the neural modeling literature \citep{10.1371/journal.pcbi.1006897,DBLP:conf/nips/KlindtEEB17}, we used activation layers without bound in the output (ReLU, softplus) whereas the models explored in \citet{DBLP:conf/nips/BaiKK19} mostly use activation layers with bounded output (tanh, sigmoid); we tried training some of our models using tanh or sigmoid activation layers and obtained much worse results in terms of neural prediction metrics.



\subsubsection{Alternative mechanisms of efficiently increasing the receptive field size}

% connection with other work for increased RF size.
From a computational perspective, among other things, our recurrent models increase the effective receptive field size of output units via lateral recurrent connections. In the machine learning community, alternative approaches such as non-local neural networks \citep{DBLP:conf/cvpr/0004GGH18} and self-attention \citep{DBLP:conf/nips/VaswaniSPUJGKP17} can also effectively increase the receptive field size of output units with efficiency in model size. It will be interesting to compare recurrent networks with these alternative approaches in the neural data modeling domain.

\subsection{Limitations and future work}

\subsubsection{True recurrent dynamics versus semi-recurrent dynamics with shared convolutional layers and independent normalization layers}
\label{nips2021:discussions:limitation:strict_recurrent}

As noted in Sections~\ref{method:new},\ref{appendix:model_math:new}, For our recurrent models, batch normalization is applied independently across time, following \citet{10.1371/journal.pcbi.1008215}. While this means that our models are not truly recurrent due to the independent normalization layer at each time step, our main conclusion that (semi-) recurrent models outperformed feed-forward models of matched size and hyperparameters still held (Section~\ref{results:datadriven_models}), as independent batch normalization layers add less than 1\% to the overall model size, whereas increasing the number of channel or any other hyparparameter (kernel size, number of layers, etc.) by one generally induces an increase of model size of greater than or equal to 5\%; in other words, model size increase cannot explain the performance advantage of our recurrent models over feed-forward ones. In addition, many other studies \citep{DBLP:conf/nips/KubiliusSHMRIKB19,DBLP:conf/nips/HanWZFCL18,10.1371/journal.pcbi.1008215} that apply recurrent models to neural modeling or computer vision tasks have used independent normalization layers across time as well, potentially in order to address stability issues in model optimization. 

\subsubsection{Relative versus absolute performance gain of recurrent models}

While recurrent models consistently outperformed feed-forward models matched in model size and hyperparameters, the absolute performance increase was still modest, compared to the amount of variance yet to be explained in the neural data. Adding feedback recurrent connections to our models that only contain lateral recurrent connections, exploring alternative readout modes (Section~\ref{method:new:readout}), and exploring other basic network components rather than convolution might help to fully capture the neural computation of early visual areas.

\subsubsection{Connection of our work to the brain}

We did not try to map the recurrent circuits in our best-performing models to the biological recurrent circuits in the brain. In general, given the nonconvex nature of neural networks, all recurrent neural network architectures in general might be equivalent in terms of performance  given sufficient hyparparameter tuning \citep{DBLP:conf/iclr/CollinsSS17}. However, it's likely that recurrent circuits benefit the brain in the same way as they benefit our models; in particular, biological recurrent circuits form compact and implicit multi-path ensembles that allow the brain to learn complex neural responses to visual stimuli with data efficiency. Given that we demonstrated the advantage of recurrent models consistently in two data sets with different stimulus presentation paradigms (Section~\ref{method:data}) in modeling mean firing rates instead of temporal dynamics (Section~\ref{nips2021:discussion:relationship:dynamics}), it's likely that our recurrent circuits capture some general aspects about neural computation in the early visual areas rather than any specific circuits of the brain.

To better map the recurrent circuits in the model to those in the brain, additional metrics other than neural data prediction under natural stimuli can be used for model comparison. For example, \citet{DBLP:conf/nips/KubiliusSHMRIKB19} leveraged existing knowledge about brain anatomy to constrain the number of layers in their recurrent models, and \citet{10.3389/fpsyg.2017.01551,Rajaei302034} justified the validity their recurrent models by comparing model prediction and neural data under occluded object recognition tasks; in addition, neurophysiological experiments can be performed on models to see if they can produce various neural response properties (surround suppression, end-stopping, etc.) thought to be related to recurrent circuits \citep{Zhu:2013fi}. Preliminary results in \citet{halcosyne2021} showed that the internal model dynamics of our recurrent models exhibited longitudinal facilitation and lateral suppression of oriented bars \citep{Kapadia12073} as well as reduction in orientation bandwidths and spatial frequency bandwidths over time \citep{ringach1997dynamics,Bredfeldt1976}.

Regarding the connection between the brain and neural network-based methods as a whole, there have been numerous studies comparing CNNs with biological data at the neural level, at the behavior level, and from many other aspects \citep{doi:10.1162/jocn_a_01544}; while there are still many inconsistencies between CNNs and the biogloical visual system, generally speaking for now CNNs can be considered a viable model for the brain.

\subsubsection{Testing the reformulation method in other machine learning contexts}

Our novel reformulation method  provides a new perspective to understand recurrent models and connect recurrent models to the existing literature on ensemble models. As discussed in the end of Section~\ref{nips2021:discussion:contribution}, applying our reformulation method and analysis techniques to other recurrent model-related studies, such as  architecture search studies \citep{DBLP:conf/iclr/CollinsSS17,DBLP:journals/corr/GreffSKSS15} for recurrent models as well as computer vision studies \citep{nayebi2018task,DBLP:conf/nips/KubiliusSHMRIKB19,DBLP:conf/nips/HanWZFCL18} involving recurrent models, might yield additional insights on the advantage of recurrent computation for machine learning tasks in general.


